Readie: Low-Latency Code Sandboxes for AI Agents

From quantitative research to personal assistance, AI agents act by iteratively generating and executing code. To decouple the agent harness from code execution, many agents offload execution to dedicated systems called code sandboxes. However, existing code sandboxes suffer from slow startup. Whether they rely on custom snapshots or a single fat image, the root cause is the same: it is hard to build a compact, pre-warmed snapshot that can be shared across diverse agent-generated code while covering nearly all the artifacts (e.g., packages, datasets) it requires. In this work, we propose learned startup snapshots for low-latency code sandboxes. Our insight is that while it is hard for a single snapshot to be both compact and cover most workloads, a set of snapshots can achieve both. Each snapshot is small, initializes quickly, and covers a fraction of agent-generated code; together, the set covers most of it. We learn this set from a large training workload by formulating snapshot construction as an optimization problem and solving it with an approximation algorithm. Planned on 15K public and LLM-synthesized scripts, our system, Readie, reduces startup latency by 3-22$\times$ and end-to-end runtime by 1.3-3.3$\times$ compared to existing approaches at the same storage budget.

==> figures/alpha_data.tex <==
\def\alAlpha{0.0031}% s per MB
\def\alBase{0.32}% s
\def\alN{50}%
\def\alXmax{800}\def\alYmax{3.5}%


==> figures/domain_residual_data.tex <==
% Generated by experiments/analysis/export_tex.py. Do not edit.
\def\drTicks{0.0000,0.2000,0.4000,0.6215,0.7734,0.9253}
\def\drTickLabels{0,400,800,5k,10k,15k}
\def\drBreak{0.5}
\def\drCoords{{Time Series Analysis}, {Graph Processing}, {Natural Language Processing}, {Computer Vision}, {Model Training \& Inference}, {Exploration \& Visualization}, {Data Preparation}, {Machine Learning}}
\def\drRows{8}


==> figures/fig_architecture_offline.tex <==
% The offline pipeline that builds the checkpoints, left to right: planning data,
% metadata generation, planning checkpoint sets, checkpoint creation.
% Panel (b) of the architecture figure; panel (a) is fig_architecture.tex.
% One column wide. Use: \input{figures/fig_architecture_offline.tex}. No data file.
\begingroup
\definecolor{soOffline}{RGB}{232,232,232}%
\tikzset{
  so stage/.style={draw, rounded corners=2pt, fill=soOffline, font=\scriptsize, align=center,
    minimum width=1.75cm, minimum height=9mm, inner sep=1.5pt},
  so arr/.style={-latex, semithick},
}%
\begin{tikzpicture}[x=1cm,y=1cm]
  \foreach \i/\x/\txt in {1/0.875/{Planning\\data},2/3.02/{Metadata\\generation},
                          3/5.165/{Planning\\snapshot sets},4/7.315/{Snapshot\\creation}}
    \node[so stage] (sooff\i) at (\x,0) {\txt};
  \foreach \i/\j in {1/2,2/3,3/4}
    \draw[so arr] (sooff\i) -- (sooff\j);
\end{tikzpicture}%
\endgroup


==> figures/fig_latency_hist.tex <==
% Latency histograms, one row of four panels (one per method), with p50/p90/p95/p99 marked. Shared body
% of the fig_methods_* wrappers, which set \lhSet (test|agent), \lhMetric (init|e2e) and \lhXlabel first;
% \lhKey draws the key of the rules above the row, \lhNames the methods' names below it.
% Use: \input{figures/fig_methods_test_init.tex} inside a figure*; needs \usepackage{pgfplots}.
% Data: figures/hist_<set>_<metric>.dat and figures/latency_hist_data.tex, written by experiments/methods/export_tex.py.
\begingroup
\ifdefined\lhWidth\else\def\lhWidth{3.5cm}\fi% four panels and their gaps fill \textwidth
\def\lhGap{0.65cm}% between panels, room for the next panel's y tick labels
\input{figures/latency_hist_data.tex}%
\definecolor{lhNockpt}{HTML}{6D6C67}%
\definecolor{lhFat}{HTML}{EB6834}%
\definecolor{lhPrmin}{HTML}{2A78D6}%
\definecolor{lhBounded}{HTML}{1BAF7A}%
\definecolor{lhInk}{HTML}{52514E}%
\def\lhv#1#2{\csname lh-\lhSet-\lhMetric-#1-#2\endcsname}%
% the same scale in every figure (1.14cm for 30%), so a lower ceiling gives a shorter panel
\pgfmathsetlengthmacro\lhHeight{0.038cm*\csname lh-\lhSet-\lhMetric-ymax\endcsname}%
\pgfplotsset{
  lh panel/.style={
    width=\lhWidth, height=\lhHeight, scale only axis,
    xmin=\csname lh-\lhSet-\lhMetric-xmin\endcsname, xmax=\csname lh-\lhSet-\lhMetric-xmax\endcsname, ymin=0, ymax=\csname lh-\lhSet-\lhMetric-ymax\endcsname,
    ytick={0,\csname lh-\lhSet-\lhMetric-ymax\endcsname},
    ticklabel style={font=\scriptsize}, label style={font=\scriptsize},
    axis lines*=left, axis line style={lhInk}, tick style={lhInk},
    ymajorgrids, grid style={black!10, line width=0.3pt},
    xminorticks=false, clip=false,
  },
}%
% \lhRule{key}{percentile}{dash style}
\def\lhRule#1#2#3{\draw[lhInk, line width=0.5pt, #3]
  (axis cs:\lhv{#1}{#2}, 0) -- (axis cs:\lhv{#1}{#2}, {\csname lh-\lhSet-\lhMetric-ymax\endcsname});}%
% \lhPanel{key}{color}{extra axis options}
\def\lhPanel#1#2#3{%
  \begin{axis}[lh panel, xmode=log, name=p#1, #3]
    \addplot[const plot, fill=#2, fill opacity=0.85, draw=#2, line width=0.2pt, forget plot]
      table[x=edge, y=#1] {figures/hist_\lhSet_\lhMetric.dat} \closedcycle;
    \lhRule{#1}{fifty}{solid}\lhRule{#1}{ninety}{dashed}\lhRule{#1}{ninetyfive}{dotted}\lhRule{#1}{ninetynine}{dashdotted}%
    \node[anchor=south east, font=\scriptsize, inner sep=1pt] at (rel axis cs:1,1)
      {\lhv{#1}{fifty} \enspace \lhv{#1}{ninety} \enspace \lhv{#1}{ninetyfive} \enspace \lhv{#1}{ninetynine}\,s};
  \end{axis}}%
% \lhName{key}{label}: the method's name, centred below its panel and the axis label
\def\lhName#1#2{\node[anchor=north, font=\scriptsize\bfseries, inner sep=1pt] at ([yshift=-2pt]p#1.south |- lhx.south) {#2};}%
\begin{tikzpicture}
  \lhPanel{nockpt}{lhNockpt}{}
  \lhPanel{fat}{lhFat}{at={(pnockpt.south east)}, anchor=south west, xshift=\lhGap}
  \lhPanel{prmin}{lhPrmin}{at={(pfat.south east)}, anchor=south west, xshift=\lhGap}
  \lhPanel{bounded}{lhBounded}{at={(pprmin.south east)}, anchor=south west, xshift=\lhGap}
  \coordinate (lhmid) at ($(pnockpt.south west)!0.5!(pbounded.south east)$);
  \node[anchor=north, font=\scriptsize, inner sep=1pt] (lhx) at ([yshift=-1pt]lhmid |- pnockpt.outer south) {\lhXlabel};
  % the names of the methods, once, under the bottom row (\lhNames)
  \ifdefined\lhNames
    \lhName{nockpt}{No snapshots}\lhName{fat}{Fat image}\lhName{prmin}{Per-request (8\,GB)}\lhName{bounded}{\sys (10\,GB) (ours)}
  \fi
  \node[font=\scriptsize, rotate=90, anchor=south] at ([xshift=-0.5cm]$(pnockpt.south west)!0.5!(pnockpt.north west)$) {\% of requests};
  % key: the four rules; the numbers above each panel are the four percentiles in seconds, in this order
  \ifdefined\lhKey
  \node[anchor=south, font=\scriptsize, inner sep=0pt] at ([yshift=0.45cm]lhmid |- pnockpt.north)
    {\tikz[baseline=-0.5ex]{\draw[lhInk, line width=0.5pt] (0,0)--(0.22,0);}\,p50\hspace{0.6em}
     \tikz[baseline=-0.5ex]{\draw[lhInk, line width=0.5pt, dashed] (0,0)--(0.22,0);}\,p90\hspace{0.6em}
     \tikz[baseline=-0.5ex]{\draw[lhInk, line width=0.5pt, dotted] (0,0)--(0.22,0);}\,p95\hspace{0.6em}
     \tikz[baseline=-0.5ex]{\draw[lhInk, line width=0.5pt, dashdotted] (0,0)--(0.22,0);}\,p99};
  \fi
\end{tikzpicture}%
\endgroup


==> figures/fig_methods_agent_e2e.tex <==
% Histogram of e2e times on the agent set (No snapshots, fat image, per-request 8 GB cache, \sys 10 GB).
% Use: \input{figures/fig_methods_agent_e2e.tex} inside a figure; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
% Body and data: see fig_latency_hist.tex.
\begingroup
\def\lhSet{agent}\def\lhMetric{e2e}\def\lhXlabel{End-to-end time (s)}%
\input{figures/fig_latency_hist.tex}%
\endgroup


==> figures/fig_methods_agent_init.tex <==
% Histogram of init times on the agent set (No snapshots, fat image, per-request 8 GB cache, \sys 10 GB).
% Use: \input{figures/fig_methods_agent_init.tex} inside a figure; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
% Body and data: see fig_latency_hist.tex.
\begingroup
\def\lhSet{agent}\def\lhMetric{init}\def\lhXlabel{Initialization time (s)}%
\input{figures/fig_latency_hist.tex}%
\endgroup


==> figures/fig_methods_agent_pair.tex <==
% Init and end-to-end histograms on the agent set stacked, init above end-to-end, across both columns.
% Use: \begin{figure*}[t]\centering\input{figures/fig_methods_agent_pair.tex}\caption{...}\end{figure*}; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
\begingroup
{\def\lhKey{}\input{figures/fig_methods_agent_init.tex}}\\[4pt]
{\def\lhNames{}\input{figures/fig_methods_agent_e2e.tex}}
\par\vspace{-4pt}% pull the figure caption closer
\endgroup


==> figures/fig_methods_test_e2e.tex <==
% Histogram of e2e times on the test set (No snapshots, fat image, per-request 8 GB cache, \sys 10 GB).
% Use: \input{figures/fig_methods_test_e2e.tex} inside a figure; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
% Body and data: see fig_latency_hist.tex.
\begingroup
\def\lhSet{test}\def\lhMetric{e2e}\def\lhXlabel{End-to-end time (s)}%
\input{figures/fig_latency_hist.tex}%
\endgroup


==> figures/fig_methods_test_init.tex <==
% Histogram of init times on the test set (No snapshots, fat image, per-request 8 GB cache, \sys 10 GB).
% Use: \input{figures/fig_methods_test_init.tex} inside a figure; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
% Body and data: see fig_latency_hist.tex.
\begingroup
\def\lhSet{test}\def\lhMetric{init}\def\lhXlabel{Initialization time (s)}%
\input{figures/fig_latency_hist.tex}%
\endgroup


==> figures/fig_methods_test_pair.tex <==
% Init and end-to-end histograms on the test set stacked, init above end-to-end, across both columns.
% Use: \begin{figure*}[t]\centering\input{figures/fig_methods_test_pair.tex}\caption{...}\end{figure*}; needs \usepackage{pgfplots} and \usetikzlibrary{calc}.
\begingroup
{\def\lhKey{}\input{figures/fig_methods_test_init.tex}}\\[4pt]
{\def\lhNames{}\input{figures/fig_methods_test_e2e.tex}}
\par\vspace{-4pt}% pull the figure caption closer
\endgroup


==> figures/fig_planners_col.tex <==
% Figs (a) planning set, (b) validation set, (c) planning time and the shared key, as a 2x2 grid in one column,
% with shorter panels and smoothed lines (\plSoft). Use: \begin{figure}\centering\input{figures/fig_planners_col.tex}\caption{...}\end{figure}.
\begingroup
\def\plWidth{2.55cm}\def\plHeight{1.25cm}\def\plNoLegend{}\def\plSoft{}%
\captionsetup[sub]{skip=1pt}% sub-captions closer to the small panels
\pgfplotsset{% fewer labelled ticks, so the small panels stay legible, with one unlabelled y tick between them
  pl ticks planner_storage_planning/.style={xtick={1,4,8,12,16,20}, ytick distance=10, minor y tick num=1},
  pl ticks planner_storage_validation/.style={xtick={1,4,8,12,16,20}, ytick distance=1, minor y tick num=1},
  pl ticks planner_time/.style={xtick distance=3000, ytick distance=100, minor y tick num=1, xlabel={Requests planned (thousands)},
    xticklabel={\pgfmathparse{\tick/1000}\pgfmathprintnumber[fixed, precision=0]{\pgfmathresult}}}}%
\definecolor{plGreedy}{HTML}{1BAF7A}\definecolor{plTop}{HTML}{6D6C67}\definecolor{plKmed}{HTML}{2A78D6}\definecolor{plJagg}{HTML}{8A5DB0}%
\def\plKey#1#2#3#4{\tikz[baseline=-0.5ex]{\draw[#1, line width=0.6pt] (0,0)--(0.45,0); \node[mark size=#4, #1] at (0.225,0) {\pgfuseplotmark{#2}};}\,\textbf{#3}}%
\begin{subfigure}[t]{0.49\columnwidth}\centering
  \input{figures/fig_planners_planning.tex}
  \subcaption{Planning set}\label{fig:planners_a}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.49\columnwidth}\centering
  \input{figures/fig_planners_validation.tex}
  \subcaption{Validation set}\label{fig:planners_b}
\end{subfigure}\\[0pt]
\begin{subfigure}[b]{0.6\columnwidth}\centering
  \def\plWidth{3.55cm}% wider than (a) and (b): the key beside it needs less room
  \input{figures/fig_planners_time.tex}
  \subcaption{Planning time}\label{fig:planners_c}
\end{subfigure}\hfill
\begin{minipage}[b]{0.39\columnwidth}\raggedleft
  {\scriptsize\begin{tabular}{@{}l@{}}
    \plKey{plGreedy}{*}{Greedy facility location}{0.8pt}\\[1pt]
    \plKey{plTop}{square*}{Greedy knapsack}{0.6pt}\\[1pt]
    \plKey{plKmed}{triangle*}{$k$-medoids}{0.8pt}\\[1pt]
    \plKey{plJagg}{diamond*}{Agglomerative Jaccard}{0.8pt}
  \end{tabular}}\par\vspace{0.75cm}
\end{minipage}
\par\vspace{-8pt}% pull the figure caption closer to the sub-captions
\endgroup


==> figures/fig_planners_legend.tex <==
% One legend line for a row of planner panels (see fig_planners_row.tex); colours and markers match fig_planners.tex.
\begingroup
\definecolor{plGreedy}{HTML}{1BAF7A}\definecolor{plTop}{HTML}{6D6C67}\definecolor{plKmed}{HTML}{2A78D6}\definecolor{plJagg}{HTML}{8A5DB0}%
\def\plKey#1#2#3{\tikz[baseline=-0.5ex]{\draw[#1, line width=0.8pt] (0,0)--(0.5,0); \node[mark size=1.3pt, #1] at (0.25,0) {\pgfuseplotmark{#2}};}\,\textbf{#3}}%
\begin{tikzpicture}
  \tikzset{every node/.style={font=\scriptsize}}
  \node[inner sep=2pt] {\plKey{plGreedy}{*}{Greedy facility location}\quad\plKey{plTop}{square*}{Greedy knapsack}\quad\plKey{plKmed}{triangle*}{$k$-medoids}\quad\plKey{plJagg}{diamond*}{Agglomerative Jaccard}};
\end{tikzpicture}%
\endgroup


==> figures/fig_planners_planning.tex <==
% Planner comparison, total time over its requests against the checkpoint budget, planning set.
% Use: \input{figures/fig_planners_planning.tex} inside a figure; needs \usepackage{pgfplots}. Body: fig_planners.tex.
\begingroup
\def\plFile{planner_storage_planning}\def\plXcol{gb}\def\plXlabel{Snapshot budget (GB)}\def\plYlabel{Total time (h)}\def\plYmax{\plStorageYmaxPlanning}\def\plCold{\plColdPlanning}\def\plXmax{20}%
\pgfplotsset{pl ticks/.style={xtick={1,2,4,6,8,10,12,16,20}, ytick distance=5}}%
\input{figures/fig_planners.tex}%
\endgroup


==> figures/fig_planners_time.tex <==
% Planner comparison, planning time against the number of data points.
% Use: \input{figures/fig_planners_time.tex} inside a figure; needs \usepackage{pgfplots}. Body: fig_planners.tex.
\begingroup
\def\plFile{planner_time}\def\plXcol{points}\def\plXlabel{Data points planned on (thousands)}\def\plYlabel{Planning time (s)}\def\plYmax{\plTimeYmax}\def\plXmax{\plTimeXmax}%
\pgfplotsset{pl ticks/.style={xtick distance=2500, ytick distance=50,
  xticklabel={\pgfmathparse{\tick/1000}\pgfmathprintnumber[fixed, precision=1]{\pgfmathresult}}}}%
\input{figures/fig_planners.tex}%
\endgroup


==> figures/fig_planners_validation.tex <==
% Planner comparison, total time over its requests against the checkpoint budget, validation set.
% Use: \input{figures/fig_planners_validation.tex} inside a figure; needs \usepackage{pgfplots}. Body: fig_planners.tex.
\begingroup
\def\plFile{planner_storage_validation}\def\plXcol{gb}\def\plXlabel{Snapshot budget (GB)}\def\plYlabel{Total time (h)}\def\plYmax{\plStorageYmaxValidation}\def\plCold{\plColdValidation}\def\plXmax{20}%
\pgfplotsset{pl ticks/.style={xtick={1,2,4,6,8,10,12,16,20}, ytick distance=0.5,
  yticklabel style={/pgf/number format/.cd, fixed, precision=1}}}%
\input{figures/fig_planners.tex}%
\endgroup


==> figures/layer_pull_data.tex <==
% Generated by experiments/layer_pull/export_tex.py (median run per case). Do not edit.
\def\lpPhasesCold{\lpPhase{2.7}{3.3}{0.07}{0.57}{lpDownload} \lpPhase{2.7}{3.3}{0.64}{2.01}{lpExtract} \lpNote{3}{2.01}{0.5\,s + 1.4\,s} \lpPhase{1.7}{2.3}{0.07}{0.40}{lpDownload} \lpPhase{1.7}{2.3}{2.01}{3.01}{lpExtract} \lpNote{2}{3.01}{0.3\,s + 1.0\,s} \lpPhase{0.7}{1.3}{0.25}{3.05}{lpDownload} \lpPhase{0.7}{1.3}{3.08}{15.24}{lpExtract} \lpNote{1}{15.24}{2.8\,s + 12.2\,s} \lpPhase{-0.3}{0.3}{15.30}{17.39}{lpRun} \lpNote{0}{17.39}{2.1\,s}}
\def\lpFetchedCold{358}
\def\lpReadyCold{17.4}
\def\lpPhasesCached{\lpCached{3} \lpCached{2} \lpPhase{0.7}{1.3}{0.16}{2.76}{lpDownload} \lpPhase{0.7}{1.3}{2.88}{14.74}{lpExtract} \lpNote{1}{14.74}{2.6\,s + 11.9\,s} \lpPhase{-0.3}{0.3}{14.77}{16.86}{lpRun} \lpNote{0}{16.86}{2.1\,s}}
\def\lpFetchedCached{312}
\def\lpReadyCached{16.9}
\def\lpCacheSaving{0.5}


==> figures/planners_data.tex <==
% Generated by experiments/algorithm/export_tex.py. Do not edit.
\def\plStorageYmaxPlanning{35.0}\def\plColdPlanning{128.0}
\def\plStorageYmaxValidation{4.5}\def\plColdValidation{16.4}
\def\plTimeYmax{300.0}
\def\plTimeXmax{15000}


==> figures/workload_clusters_areas.tex <==
% Generated by experiments/workload_clusters/export_tex.py. Do not edit.
\def\wcAreas{\wcArea{wcTab}{(axis cs:6.095,-2.337) -- (axis cs:6.461,-2.150) -- (axis cs:6.785,-1.867) -- (axis cs:7.061,-1.490) -- (axis cs:7.285,-1.028) -- (axis cs:7.452,-0.488) -- (axis cs:7.561,0.121) -- (axis cs:7.610,0.789) -- (axis cs:7.596,1.504) -- (axis cs:7.521,2.253) -- (axis cs:7.386,3.024) -- (axis cs:7.194,3.804) -- (axis cs:6.946,4.580) -- (axis cs:6.649,5.338) -- (axis cs:6.306,6.064) -- (axis cs:5.924,6.748) -- (axis cs:5.510,7.377) -- (axis cs:5.069,7.940) -- (axis cs:4.611,8.427) -- (axis cs:4.142,8.831) -- (axis cs:3.671,9.144) -- (axis cs:3.205,9.362) -- (axis cs:2.754,9.479) -- (axis cs:2.324,9.495) -- (axis cs:1.923,9.409) -- (axis cs:1.557,9.223) -- (axis cs:1.233,8.939) -- (axis cs:0.957,8.563) -- (axis cs:0.733,8.101) -- (axis cs:0.566,7.561) -- (axis cs:0.457,6.951) -- (axis cs:0.408,6.284) -- (axis cs:0.422,5.569) -- (axis cs:0.497,4.820) -- (axis cs:0.632,4.048) -- (axis cs:0.824,3.268) -- (axis cs:1.072,2.493) -- (axis cs:1.369,1.735) -- (axis cs:1.712,1.008) -- (axis cs:2.094,0.325) -- (axis cs:2.508,-0.304) -- (axis cs:2.949,-0.867) -- (axis cs:3.407,-1.354) -- (axis cs:3.876,-1.758) -- (axis cs:4.347,-2.072) -- (axis cs:4.813,-2.289) -- (axis cs:5.264,-2.407) -- (axis cs:5.694,-2.423)}
  \wcArea{wcVis}{(axis cs:10.322,4.668) -- (axis cs:10.342,4.846) -- (axis cs:10.331,5.027) -- (axis cs:10.288,5.208) -- (axis cs:10.215,5.386) -- (axis cs:10.113,5.558) -- (axis cs:9.984,5.722) -- (axis cs:9.829,5.873) -- (axis cs:9.652,6.011) -- (axis cs:9.455,6.131) -- (axis cs:9.242,6.233) -- (axis cs:9.017,6.314) -- (axis cs:8.783,6.374) -- (axis cs:8.544,6.411) -- (axis cs:8.305,6.424) -- (axis cs:8.069,6.413) -- (axis cs:7.841,6.379) -- (axis cs:7.624,6.322) -- (axis cs:7.422,6.243) -- (axis cs:7.240,6.143) -- (axis cs:7.078,6.024) -- (axis cs:6.942,5.888) -- (axis cs:6.832,5.738) -- (axis cs:6.751,5.576) -- (axis cs:6.700,5.405) -- (axis cs:6.680,5.227) -- (axis cs:6.691,5.046) -- (axis cs:6.733,4.865) -- (axis cs:6.806,4.686) -- (axis cs:6.908,4.514) -- (axis cs:7.038,4.351) -- (axis cs:7.192,4.199) -- (axis cs:7.370,4.062) -- (axis cs:7.566,3.941) -- (axis cs:7.779,3.840) -- (axis cs:8.005,3.758) -- (axis cs:8.239,3.699) -- (axis cs:8.478,3.662) -- (axis cs:8.717,3.649) -- (axis cs:8.953,3.660) -- (axis cs:9.181,3.694) -- (axis cs:9.398,3.751) -- (axis cs:9.599,3.830) -- (axis cs:9.782,3.930) -- (axis cs:9.943,4.048) -- (axis cs:10.080,4.184) -- (axis cs:10.190,4.334) -- (axis cs:10.271,4.497)}
  \wcArea{wcNlp}{(axis cs:5.883,6.721) -- (axis cs:6.115,6.805) -- (axis cs:6.332,6.928) -- (axis cs:6.530,7.089) -- (axis cs:6.706,7.285) -- (axis cs:6.857,7.513) -- (axis cs:6.981,7.768) -- (axis cs:7.074,8.047) -- (axis cs:7.137,8.344) -- (axis cs:7.167,8.654) -- (axis cs:7.164,8.973) -- (axis cs:7.128,9.294) -- (axis cs:7.060,9.613) -- (axis cs:6.961,9.923) -- (axis cs:6.832,10.219) -- (axis cs:6.676,10.497) -- (axis cs:6.496,10.751) -- (axis cs:6.294,10.978) -- (axis cs:6.074,11.173) -- (axis cs:5.840,11.333) -- (axis cs:5.595,11.455) -- (axis cs:5.345,11.538) -- (axis cs:5.093,11.579) -- (axis cs:4.843,11.578) -- (axis cs:4.600,11.536) -- (axis cs:4.369,11.452) -- (axis cs:4.152,11.328) -- (axis cs:3.953,11.167) -- (axis cs:3.777,10.971) -- (axis cs:3.626,10.743) -- (axis cs:3.503,10.488) -- (axis cs:3.409,10.210) -- (axis cs:3.346,9.913) -- (axis cs:3.316,9.602) -- (axis cs:3.319,9.284) -- (axis cs:3.355,8.962) -- (axis cs:3.423,8.644) -- (axis cs:3.523,8.334) -- (axis cs:3.651,8.037) -- (axis cs:3.807,7.760) -- (axis cs:3.988,7.505) -- (axis cs:4.190,7.278) -- (axis cs:4.409,7.084) -- (axis cs:4.644,6.923) -- (axis cs:4.888,6.801) -- (axis cs:5.138,6.719) -- (axis cs:5.390,6.678) -- (axis cs:5.640,6.678)}}
\def\wcCkpts{\wcCkpt{wcTab}{1}{3.793}{4.966}
  \wcCkpt{wcVis}{2}{8.156}{5.224}
  \wcCkpt{wcNlp}{3}{4.480}{9.511}}


==> figures/workload_clusters_labels.tex <==
% Generated by experiments/workload_clusters/export_tex.py. Do not edit.
\def\wcLabels{\wcLabel{4.480}{9.511}{-0.35}{9.511}{east}{right}{\textcolor{black}{\textbf{$\bm{c_3}$:} }\textcolor{black}{\textbf{numpy, pandas,}}\\\textcolor{black}{\textbf{transformers}}}
  \wcLabel{4.894}{8.221}{-0.35}{6.841}{east}{right}{\textcolor{wcInk}{matplotlib,}\\\textcolor{wcInk}{numpy, pandas,}\\\textcolor{wcInk}{scikit-learn,}\\\textcolor{wcInk}{seaborn,}\\\textcolor{wcInk}{transformers}}
  \wcLabel{3.793}{4.966}{-0.35}{3.451}{east}{right}{\textcolor{black}{\textbf{$\bm{c_1}$:} }\textcolor{black}{\textbf{matplotlib,}}\\\textcolor{black}{\textbf{numpy, pandas,}}\\\textcolor{black}{\textbf{scikit-learn,}}\\\textcolor{black}{\textbf{seaborn}}}
  \wcLabel{4.500}{1.678}{-0.35}{0.781}{east}{right}{\textcolor{wcInk}{keras, numpy,}\\\textcolor{wcInk}{pandas,}\\\textcolor{wcInk}{scikit-learn}}
  \wcLabel{3.967}{8.082}{10.6}{8.082}{west}{left}{\textcolor{wcInk}{matplotlib,}\\\textcolor{wcInk}{numpy, pandas,}\\\textcolor{wcInk}{scikit-learn,}\\\textcolor{wcInk}{torch}}
  \wcLabel{9.000}{5.990}{10.6}{5.412}{west}{left}{\textcolor{wcInk}{matplotlib,}\\\textcolor{wcInk}{numpy, pillow,}\\\textcolor{wcInk}{scikit-learn}}
  \wcLabel{8.156}{5.224}{10.0}{2.022}{west}{left}{\textcolor{black}{\textbf{$\bm{c_2}$:} }\textcolor{black}{\textbf{matplotlib,}}\\\textcolor{black}{\textbf{numpy,}}\\\textcolor{black}{\textbf{opencv-python,}}\\\textcolor{black}{\textbf{pandas, pillow,}}\\\textcolor{black}{\textbf{scikit-learn,}}\\\textcolor{black}{\textbf{seaborn}}}}

